How Do Programming Students Use Generative AI?

Programming students have a widespread access to powerful Generative AI tools like ChatGPT. While this can help understand the learning material and assist with exercises, educators are voicing more and more concerns about an overreliance on generated outputs and lack of critical thinking skills. It is thus important to understand how students actually use generative AI and what impact this could have on their learning behavior. To this end, we conducted a study including an exploratory experiment with 37 programming students, giving them monitored access to ChatGPT while solving a code authoring exercise. The task was not directly solvable by ChatGPT and required code comprehension and reasoning. While only 23 of the students actually opted to use the chatbot, the majority of those eventually prompted it to simply generate a full solution. We observed two prevalent usage strategies: to seek knowledge about general concepts and to directly generate solutions. Instead of using the bot to comprehend the code and their own mistakes, students often got trapped in a vicious cycle of submitting wrong generated code and then asking the bot for a fix. Those who self-reported using generative AI regularly were more likely to prompt the bot to generate a solution. Our findings indicate that concerns about potential decrease in programmers' agency and productivity with Generative AI are justified. We discuss how researchers and educators can respond to the potential risk of students uncritically over-relying on Generative AI. We also discuss potential modifications to our study design for large-scale replications.

==> sections/2background.tex <==
% Background & related work

\section{Background}\label{background}

A significant push towards the emergence of current-day \llms can be attributed to the Generative Pre-trained Transformer (GPT) family of language models \cite{B20_GPT3, O23_GPT4, R18_GPT, R19_GPT2}.
These models are Transformers that have been trained on large unlabeled corpora of documents, articles, books and other sources from the web (see \eg WebText \cite{B20_GPT3, R19_GPT2}) for the task of generating text.
A user-provided string, commonly referred to as a \textit{prompt} (see \eg \cite{B20_GPT3, R19_GPT2}), can be used as the initial input, to which the model generates text that is considered likely to follow.
Each time the model generates a token (roughly equivalent to a single word \cite{S15_BPE}), it becomes part of the input sequence for the following generation steps, thus disallowing the model from backtracking over its own output. \cite{R18_GPT}
%Text is divided up into tokens (words or sub-word units, see \eg \cite{S15_BPE}).
%An individual generation step then takes the existing tokens as input and predicts a single token that is likely to follow from the given context.
%They can then be used to generate new text one token\footnote{Tokens are atomic word or sub-word units that the language models represent text with, as vectors in an embedding space. In the case of \gptv{2} and \gptv{3}, Byte-Pair Encoding \cite{S15_BPE} is used for tokenization.} at a time.
%At a high level, the model considers all preceding tokens and selects the token with the highest probability as the next token to generate, then repeats this process until either a maximum text length is reached or the likeliest token is a special end-of-text symbol.
%This process is repeated multiple times to generate entire text blocks.
%Each time a token is generated, it becomes part of the input sequence for the following generation steps. \cite{R18_GPT}
%This string is commonly referred to as a \textit{prompt} (see \eg \cite{B20_GPT3, R19_GPT2}).

% \paragraph{} % O22_ChatGPT
With OpenAI's release of \cgpt \cite{O22_ChatGPT} in 2022, the technology attained media attention and subsequent awareness among the general population \cite{D23_Popular}.
%Secondly, it used a supervised learning approach called \rlhf, in which human trainers were used to fine-tune a \gpt model on chat conversations between a user and the \gai system \cite{O22_ChatGPT}.
Using a supervised learning approach with data from human trainers, it was fine-tuned on conversational interactions between a user and the \llm \cite{O22_ChatGPT}.

% \paragraph{} %C21_Codex
2021 marked the release of Codex \cite{C21_Codex}, a language model specifically trained for the purpose of code generation.
In the paper, Chen et al. present the results of evaluating Codex on 164 ``hand-written programming problems'' \cite[p. 4]{C21_Codex} with unit tests.
They emphasize the need for the programming problems to be written from scratch, as opposed to collecting them from GitHub repositories or similar sources, to ensure that the problems have not been included in the training dataset for the model. \cite{C21_Codex}
